Causal Discovery with Fewer Conditional Independence Tests

Many questions in science center around the fundamental problem of understanding causal relationships. However, most constraint-based causal discovery algorithms, including the well-celebrated PC algorithm, often incur an exponential number of conditional independence (CI) tests, posing limitations in various applications. Addressing this, our work focuses on characterizing what can be learned about the underlying causal graph with a reduced number of CI tests. We show that it is possible to a learn a coarser representation of the hidden causal graph with a polynomial number of tests. This coarser representation, named Causal Consistent Partition Graph (CCPG), comprises of a partition of the vertices and a directed graph defined over its components. CCPG satisfies consistency of orientations and additional constraints which favor finer partitions. Furthermore, it reduces to the underlying causal graph when the causal graph is identifiable. As a consequence, our results offer the first efficient algorithm for recovering the true causal graph with a polynomial number of tests, in special cases where the causal graph is fully identifiable through observational data and potentially additional interventions.

==> backup/misc.tex <==
\section{Misc}

\subsection{part -1}

\begin{proof}
    We first show that $S'$ returned by Algorithm~\ref{alg:prefix_subset} satisfies $\src(\bar{S})\subset S'$. By Lemma~\ref{lem:src-not-in-Ds}, we have $\src(\bar{S})\subset U$. Then by Lemma~\ref{lem:main-lem}, we have $\src(\bar{S})\subset U'$. Thus $\src(\bar{S})\subset S'$. 

    Next we show that $S'$ is a prefix vertex set. We have $\bar{S'}=D_S\cup_{v,w'\in U} (E_v\cup F_{v,w'})$. To show that $S'$ is prefix vertex set, we only need to show that $\forall w\in \bar{S'}$ and $y\in\Des(w)$, there is $y\in \bar{S'}$. Consider the following scenarios:
    \begin{itemize}
        \item if $w\in D_S$, by Lemma~\ref{lem:Ds-has-all-des}, we know $y\in\Des(w)\subset D_S\subset \bar{S'}$.
        \item if $w\in E_v$ for some $v\in U$, we will show $y\in E_v\cup F_{v,w}$. Note that as $v\not\CI w\mid S$, there is an active path between $v,w$ given $S$. Consider extending this path by the directed path from $w$ to $y$. Note that none of vertex on the directed path from $w$ to $y$ is in $S$, as $S$ is prefixed. Therefore this extended path is also active given $S$, which means $v\not\CI y\mid S$. Thus, if $y\not\in E_v$, then there must be $u\not\CI y\mid S\cup\{v\}$. This means there is a active path, denoted by $P$, between $u$ and $y$ given $S\cup\{v\}$. If $P$ is active given $S\cup\{v,w\}$, then we have $u\not\CI y\mid S\cup\{v,w\}$, thus proving $y\in F_{v,w}$. If $P$ is inactive given $S\cup\{v,w\}$, as $P$ is active given $S\cup\{v\}$, vertex $w$ must be a non-collider on $P$. Then the path by cutting out $w$ to $y$ on $P$ is an active path between $u$ and $w$ given $S\cup\{v\}$. This contradicts $u\CI w\mid S\cup\{v\}$ as $w\in E_v$.
        \item if $w\in F_{v,w'}$ for some $v,w'\in U$, we will show $y\in F_{v,w'}$. As $w\in F_{v,w'}$, by Lemma~\ref{lemma:v-generalization}, we know $w'\not\in\Des[w]$. If $y\not\in F_{v,w'}$, then $u\CI w'\mid S\cup\{v,y\}$. Since $u\CI w'\mid S\cup\{v\}$ and $u\not\CI w'\mid S\cup\{v,w\}$, there is a path $P$ between $u,w'$ that is active given $S\cup\{v,w\}$ but inactive given $S\cup\{v\}$ or $S\cup\{v,y\}$. These mean that (1) $y$ is a non-collider on $P$, (2) all colliders on $P$ are in $\Anc[S\cup\{v,w\}]$, (3) $P$ has a collider that is in $\Anc[w]\setminus\Anc[S\cup \{v\}]$. Note that $w'\not\in\Des[y]$ as $y\in\Des[w]$ but $w'\not\in\Des[w]$, and $u\not\in\Des[w]$ as $u$ is in the prefix vertex set $S$ but $w\in\bar{S}$. Therefore $y$ being a non-collider on $P$ means there is a collider $x$ on $P$ such that $y\in\Anc(x)$. Note that this collider has to be in $\Anc[S\cup\{v,w\}]$. However as $y\not\in \Anc[S\cup\{w\}]$ and $y\in\Anc(x)$, there must be $x\in \Anc[v]$, which means $y\in\Anc(v)$. As $y\in\Des(w)$, this means $v\in\Des(w)$, which makes $\Anc[w]\setminus\Anc[S\cup \{v\}]=\varnothing$. This violates (3) above. A contradiction.
    \end{itemize}
Therefore $S'$ must be a prefix vertex set. We now bound the number of CI tests performed by Algorithm~\ref{alg:prefix_subset}: computing $D_{v,S}$ takes $O(n^2)$ CI tests; computing $E_v$ takes $O(n^2)$ CI tests; computing $F_{v,w'}$ takes $O(n^2)$ CI tests. In total, these sum up to be $O(n^4)$ CI tests.
\end{proof}

\begin{lemma}\label{lem:Ds-has-all-des}
    For each $S\subseteq V$ and $v\in\bar{S}$, if $w\in D_{v,S}$, then $\Des[w]\subseteq D_{v,S}$. Therefore if $w\not\in D_S$, there must be $\Anc[w]\cap D_S=\varnothing$.
\end{lemma}

\begin{proof}
    Since $w\in D_{v,S}$, there exists a vertex $u\in V$ such that $u \CI v\mid S$ and $u \not\CI v\mid S\cup\{w\}$. We now show that for any $x\in \Des[w]$, there is $u \not\CI v\mid S\cup\{x\}$.

    As $u \not\CI v\mid S\cup\{w\}$, there is a path $P$ from $u$ to $v$ that is active given $S\cup\{w\}$. Therefore all non-colliders on $P$ are not in $S\cup\{w\}$ and all colliders on $P$ are in $\Anc[S\cup\{w\}]$. As $x\in \Des[w]$, all colliders on $P$ are in $\Anc[S\cup\{x\}]$. If all non-colliders are not in $S\cup\{x\}$, then $P$ is the active path from $u$ to $v$ given $S\cup\{x\}$. There is $u \not\CI v\mid S\cup\{x\}$. Otherwise there is a non-collider on $P$ that is $x$.

    As $u\CI v\mid S$, path $P$ is inactive given $S$. From above we know that all non-colliders on $P$ are not in $S$. Therefore there exists a collider on $P$ that is not in $\Anc[S]$. Suppose the leftmost and rightmost such colliders are $k,k'$ (it is possible that $k=k'$), then $k,k'$ must be in $\Anc[w]\subset\Anc[x]$. Consider the path $Q$ by cutting out the parts between $k----x$ (and $k'----x$) on $P$ and replacing them with directed edges from $k$ to $x$ (and from $k'$ to $x$). Compared to $P$, the additional non-colliders on $Q$ are all on the directed path from $k$ to $x$ (or $k'$ to $x$), which are not in $S$ as $k,k'\notin \Anc[S]$. Therefore $Q$ has no non-colliders in $S$. 
    
    Compared to $P$, there is no collider on $P$ that is not in $\Anc[S]$ that is still on $Q$ by the fact that $k,k'$ are leftmost and rightmost. Therefore $x$ must be a collider on $Q$, or else $Q$ is active given $S$ and $u\not\CI v\mid S$. Therefore all non-colliders on $Q$ are not in $S\cup\{x\}$. Every collider on $Q$ is either $x$ or a collider of $P$, which is in $\Anc[S\cup\{x\}]$. Thus $Q$ is active given $S\cup\{x\}$. Therefore $u\not\CI v\mid S\cup \{x\}$.
\end{proof}

% \begin{lemma}\label{lem:one-node-anc-src}
%     Let $S$ be a prefix subset, then any $w \in \bar{S} \backslash D_{S}$ satisfies the following,
%             $$|\Anc[w] \cap \src(\bar{S})| =1~.$$
% \end{lemma}

\begin{lemma}\label{lem:src-not-in-Ds}
    Let $S$ be a prefix subset and $D_{S} = \cup_{v \in \bar{S}} D_{v,S}$, then 
    $$\src(\bar{S}) \subseteq V \backslash (S \cup D_{S})=\bar{S} \backslash D_{S}~.$$
    \kk{Need a slightly weaker statement than this, which is $\src(\bar{S}) \cap V \backslash (S \cup D_{S}) \neq \varnothing~.$}
\end{lemma}
\begin{proof}
    We prove the lemma using proof by contradiction strategy. For contradiction assume that there exists a vertex $a \in \src(\bar{S})$ such that $a \not \in \bar{S} \backslash D_{S}$, that is $a \in D_{v,S} \cap \src(\bar{S})$ for some vertex $v \in \bar{S}$. As $a \in D_{v,S}$, by the definition of the set $D_{v,S}$ there exists a vertex $u \in V$ such that, $v \CI u|S \text{ and } v \not \CI u|S \cup \{a\}$.

    As $v \CI u|S \text{ and } v \not \CI u|S \cup \{a\}$, there exists a path $P$ between $v$ and $u$ which is inactive when conditioned on $S$ but is active upon conditioning on $S \cup \{ a\}$. Moreover this path contains a vertex $b$ that is collider on $P$ and satisfies: $a \in \Des[b]$ and $\Des[b] \cap S=\varnothing$. As $\Des[b] \cap S=\varnothing$, we have that $b \in \bar{S}$. Furthermore since $b \in \bar{S}, a \in \src(\bar{S})$ and $a \in \Des[b]$, this implies that $b=a$. Therefore the path $P$ takes the form: $P=v \dots \to a \gets \dots u$. 

    All the colliders on the path $P$ either belong to or have descendant the set $S \cup \{ a\}$. 
    
    Now consider the path $v \dots \to a$ and note that it is active given $S$ because all the colliders on this path. Let $k$ be the number of vertices between $v$ and $a$ on this path $v-v_1\dots v_k\to a$. It is immediate that $v_{k} \in S$ as $a \in \src(\bar{S})$. However as $v_k \in S$, and as we condition on the set $S$, this should be collider for the path $Q$ to be active, which is not possible. Therefore a contradiction and the conclusion holds.
\end{proof}



Set $S=\varnothing$ in the above lemma we immediately have:

\begin{corollary}
    If there is no covered edge in from $\src(V)$ to $V\setminus D_\varnothing$, then $\src(V)= V \backslash D_{\varnothing}$.
\end{corollary}


\subsection{Proof of Theorem~\ref{thm:prefix-subset-int}}
\thmprefixsubsetint*

\begin{proof}
    We first prove that Algorithm~\ref{alg:prefix_subset_int} outputs a prefix vertex set. For this, note that
    \[
    \bar{S'} = D_S\cup_{v,w' \in U} (E_{v}\cup F_{v,w'})\cup_{I\in\cI} J_S^I.
    \]
    To show $S'$ is prefix, one need only to show $\forall w\in\bar{S'}$ and $y\in\Des(w)$, there is $y\in\bar{S'}$. In Theorem~\ref{thm:prefix-subset}, we have proven this for $w\in D_S\cup_{v,w' \in U} (E_{v}\cup F_{v,w'})$. Therefore we only need to consider the case where $w\in J_S^I$ for some $I\in\cI$. Invoking Lemma~\ref{lem:J-S-I}, we immediately have $y\in J_S^I$.  Thus $\bar{S'}$ is a prefix vertex set.

    Next we show that $\src(\bar{S})\subset S'$. By Theorem~\ref{thm:prefix-subset}, we have $\src(\bar{S})\cap\big(D_S\cup_{v,w' \in U} (E_{v}\cup F_{v,w'})\big)=\varnothing$. By Lemma~\ref{lem:J-S-I}, we have $\src(\bar{S})\cap \big(\cup_{I\in\cI} J_S^I\big)=\varnothing$. Thus $\src(\bar{S})\subset S'$.

    Finally we bound the number of performed CI tests. For each $I\in \cI$, computing $J_S^I$ requires computing $\Des(I\setminus S)$ and $H_S^I(v)$ for each $v\in I\setminus S$. By Lemmas~\ref{lem:des-I-S} and \ref{lem:d-v-I}, computing $\Des(I\setminus S)$ can be done in $\cO(n^2)$ CI tests. Computing each $H_S^I(v)$ is $\cO(n)$. Therefore computing $J_S^I$ for all $I\in\cI$ is bounded by $|\cI|\cdot\cO(n^2)$. Then the steps following this require at most $\cO(n^4)$ by Theorem~\ref{thm:prefix-subset}. Thus, the total number of CI test is bounded by $\cO(n^4)+|\cI|\cdot\cO(n^2)$.
\end{proof}







\subsection{part zero}

\begin{lemma}
    Let $S$ be a prefix subset and $u \in V$, $v \in \bar{S}$ and $a \in \src(\bar{S})$ be such that, $u \ci v|S$ and $u \not \ci v|S \cup \{ a\}$. Let $P$ be any active path between $u$ and $v$ when conditioned on $S \cup \{ a\}$, then all the colliders on the path $P$ belong to the set $S \cup \{ a\}$.
\end{lemma}

\begin{proof}  
Since $P$ is active given $S\cup\{a\}$, all its colliders have descendant in $S\cup\{a\}$. By $\Anc[S\cup\{a\}]\subseteq S\cup\{a\}$, we have our result.
\end{proof}

% \begin{assumption}[Single-Node Interventional Faithfulness]\label{ass:single-node-int}
%     For single-node intervention on $v\in V$, assume $P(u)\neq P^{v}(u)$ for $u\in \Des(v)$.
% \end{assumption}

% \begin{lemma}[Invariance Test]
%     Given intervention on $v\in V$, we have $P(u)\neq P^v(u)$ if and only if $u\in \Des[v]$.
% \end{lemma}

% \begin{proof}
%     If direction is provided by Assumption~\ref{ass:single-node-int}. Only if direction is provided by Markov factorization.
% \end{proof}











\subsection{part one}

\begin{lemma}
    Let $u$ and $v$ be uncomparable, then the following two statements hold,
    \begin{enumerate}
        \item $u$ is not adjacent to $v$. Therefore
        there exists a set $S \subseteq V$ such that, $u \CI v|S$.
        \item Suppose $w \in \Des(u) \cap \Des(v)$, then $u\not \CI v|S \cup w$ for all $S \subseteq V$ such that $u \CI v|S$.
    \end{enumerate}
\end{lemma}

\begin{lemma}
    If $u \CI v|\varnothing$, then $\Anc(u) \cap \Anc(v)=\varnothing$.
\end{lemma}

\begin{definition}
We call $S \subseteq V$ a prefix subset if it satisfies: for all $w \in S$, $\Anc[w] \cap \Bar{S} =\varnothing$ (Basically vertices in $S$ appear first in the order)    
\end{definition}

\begin{lemma}
    Let $S \subseteq V$ be a prefix subset. Suppose there exists a vertex $u \in \Bar{S}$ such that $u \not \sim S$, then $v \CI v|\varnothing$ for all $v\in S$ and $\Anc[v] \cap S=\varnothing$ ($v$ is not comparable to any vertex in $S$).
\end{lemma}

\paragraph{Class 1 immoralities:} $u \not\sim v$ is a class 1 immorality if and only if $u\to w\gets v$ for some $w$ and $\Anc[u]\cap\Anc[v]=\varnothing$.

\paragraph{Class 2 immoralities:} $u \not\sim v$ is a class 2 immorality if and only if $u\to w\gets v$ for some $w$ and $\Anc[u]\cap\Anc[v]\neq\varnothing$.

Let $G$ be the true DAG. Let $\Bar{G}$ be the DAG obtained from $G$ by adding edges between two vertices that satisfy Class 2 immorality.

\begin{lemma}
We can obtain $\Bar{G}$ in polynomial independence tests.
\end{lemma}

Let $F=E(\Bar{G}) \backslash E(G)$ be the set of fake edges.


\paragraph{Algorithm:} We define $I_{U}=\{(u,v)~|~u\CI v|U \}$ and $D_{U}=\{(u,v)~|~u\not \CI v|U \}$ for all $U \subseteq V$.

\begin{enumerate}
    \item Let $S=\varnothing$ denote a prefix subset. 
    \item Let $I_{S}= \{v \in \bar{S}~|~v \CI u| \varnothing \text{ for all } u\in S \}$.
    and let $I_{\varnothing}=\{(u,v)~|~u\CI v|\varnothing \}$.
    \item Let $\Bar{G}$ be recovered graph by performing independence tests conditioned on $\varnothing$ and everything.
    \item Find a source node $v_1$ of $G$ by Lemma and let $S=\{ v_1\}$ ; note that $S$ is a prefix subset.
    \item While $S \neq V$, do the following
    \begin{enumerate}
        \item If there exists a vertex $v \in V \backslash S$ such that $v$ is independent of vertices in $S$. Then by Lemma, it is not comparable to vertices in $S$ and $S \cup \{ v\}$ is a prefix subset.
        \item Else, let $I_S=\{(u,v)|u \CI v |S \}$. Let $E_{S}=\{w~|~u \CI v|S \text{ and }u \not \CI v|S\cup \{ w\} \}$. Let $F_{S}=I_{S} \backslash E_{S}$.
    \end{enumerate}
\end{enumerate}



\paragraph{Algorithm:} We define $I_{U}=\{(u,v)~|~u\CI v|U \}$ and $D_{U}=\{(u,v)~|~u\not \CI v|U \}$ for all $U \subseteq V$.

\begin{enumerate}
    \item Let $S=\varnothing$ denote a prefix subset and let $I_{\varnothing}=\{(u,v)~|~u\CI v|\varnothing \}$.
    \item Let $\Bar{G}$ be recovered graph by performing independence tests conditioned on $\varnothing$ and everything.
    \item Find a source node $v_1$ of $G$ by Lemma and let $S=\{ v_1\}$ ; note that $S$ is a prefix subset.
    \item While $S \neq V$, do the following
    \begin{enumerate}
        \item If there exists a vertex $v \in V \backslash S$ such that $v$ is independent of vertices in $S$. Then by Lemma, it is not comparable to vertices in $S$ and $S \cup \{ v\}$ is a prefix subset.
        \item Else, let $I_S=\{(u,v)|u \CI v |S \}$. Let $E_{S}=\{w~|~u \CI v|S \text{ and }u \not \CI v|S\cup \{ w\} \}$. Let $F_{S}=I_{S} \backslash E_{S}$.
    \end{enumerate}
\end{enumerate}

Let $S$ be a prefix subset. Define $A_S=\{u \in \Bar{S}~|~ \text{ there exists } v \in \Bar{S} \text{ such that } u \CI v |S \}$, $B_{S}=\{w \in \Bar{S}~|~u \CI v|S \text{ and }u \not \CI v|S\cup \{ w\} \}$ and $C_{S}=A_{S} \backslash B_{S}$. Let $N_{S}=\{v \in \Bar{S}~|~ S\cup \{ v\} \text{ is a prefix subset}\}$.

\begin{lemma}
    The following statements hold,
    \begin{enumerate}
        \item $C_{S}\neq \varnothing$ iff $S=V$. Furthermore, $N_{S} \subseteq C_{S}$.
        \item Let $u \in N_{S}$ and $w \in C_{S}$, either $w$ is not comparable to $u$ or $w \in \Des[u]$.
        \item Let $u,v \in C_{S}$, then $u \CI v~|~S$ iff $u$ and $v$ are not comparable. Therefore $C_{S}$ set can be partitioned into subsets and let $\Pt_{S}$ denote this partition of $C_{S}$ that is based on this independence test, where the elements within the same set are dependent of each other.
        \item For each element $E \in \Pt_{S}$, there exists a single source node.
        \item 
    \end{enumerate}
    
\end{lemma}

\begin{lemma}
\end{lemma}

\subsection{part two}


\paragraph{Type 1 independence tests: } Given a partially oriented graph $G(V,E,A)$, the type 1 independence checks if $u,v$ are independent.

\paragraph{Type 2 independence tests: } Given a partially oriented graph $G(V,E,A)$, the type 2 independence checks if $u,v$ are independent given $V \backslash \{u,v \}$.

\paragraph{Type 3 independence tests: } Given a partially oriented graph $G(V,E,A)$ and a vertex $w \in V$, let $R_{w}$ be the set of recovered ancestors of $w$ in $G$. The type $3$ independence test checks if $v$ is independent of $u$ given $R_{w} \cup \{w \}$.

\paragraph{Class 1 immoralities:} $u \not\sim v$ is a class 1 immorality if and only if $u\to w\gets v$ for some $w$ and $\Anc[u]\cap\Anc[v]=\varnothing$.

\paragraph{Class 2 immoralities:} $u \not\sim v$ is a class 2 immorality if and only if $u\to w\gets v$ for some $w$ and $\Anc[u]\cap\Anc[v]\neq\varnothing$.

\paragraph{Comparable vertices:} We say $u$ and $v$ are comparable if either $u \in \Des[v]$ or $v \in \Des[u]$, that is there exists a directed from either $u$ to $v$ or $v$ to $u$ in $G$.

\paragraph{Type 1 incomparable vertex pairs:} If $u$ and $v$ are incomparable and $\Anc[u] \cap \Anc[v]\neq \varnothing$, $\Des[u] \cap \Des[v]= \varnothing$.

\paragraph{Type 2 incomparable vertex pairs:} If $u$ and $v$ are incomparable and $\Anc[u] \cap \Anc[v]= \varnothing$, $\Des[u] \cap \Des[v] \neq  \varnothing$.

\paragraph{Type 3 incomparable vertex pairs:} If $u$ and $v$ are incomparable and $\Anc[u] \cap \Anc[v]\neq \varnothing$, $\Des[u] \cap \Des[v] \neq  \varnothing$.

\paragraph{Type 4 incomparable vertex pairs:} If $u$ and $v$ are incomparable and $\Anc[u] \cap \Anc[v]= \varnothing$, $\Des[u] \cap \Des[v] =  \varnothing$.

\paragraph{Type 1 comparable vertex pairs:} If $u$ and $v$ are comparable and $u$ and $v$ are adjacent.

\paragraph{Type 2 comparable vertex pairs:} If $u$ and $v$ are comparable and $u$ and $v$ are not adjacent.


\begin{lemma}
The directed edge $(u,v)$ exists in $G$ if and only if they are Type 1 comparable vertex pairs.
\end{lemma}

\begin{lemma}
    Type 1 independence test between a pair of vertices $u,v$ succeeds (that is outputs independent) if and only if $u$ and $v$ satisfy $\Anc(u) \cap \Anc(v) = \varnothing$.
\end{lemma}

\begin{lemma}
    Type 2 independence test between a pair of vertices $u,v$ succeeds (that is outputs independent) if and only if $u$ and $v$ satisfy $\Des(u) \cap \Des(v) = \varnothing$.
\end{lemma}






\paragraph{Poly number of independence tests to verify $\nu_1(\cG)=0$:} \jj{need to formalize in this case (1) all ancestral relationships $x\in\Anc(u)$ can be tested via ci tests over immorality pairs; (2) an ancestral relationship $x\in\Anc(u)$ will \emph{not} be tested via ci tests over immoralities pair that has at least one vertex \emph{not} upstream of $x$.}

The goal below is to identify $skel(\cG)$ with poly tests, then v-structures can be obtained via $\cO(n^3)$ CI tests. Then $\cG$ can be obtained through Meek rules.
\begin{itemize}
    \item identify $\cU_0$, the skeleton obtained by moralizing $\cG$, by performing type 2 independence tests for all pairs of $u,v\in V$. We have $u\sim v\in \cG_0$ if and only if $u\sim v\in \cG$ or $u\to w\gets v\in \cG$ for some $w$; in other words, $\cU_0$ contains $skel(\cG)$ and all the class 1 and 2 immoralities. 
    \item identify all the class 1 immoralities by performing type 1 independence tests for all $u\sim v\in\cU_0$. Each $u\sim v\in\cU_0$ that passes the test satisfies $u\not\sim v\in\cG$ is a class 1 immorality. Remove these edges from $\cU_0$ and obtain $\cU_1$.
    \item identify $\Des(u)\cap\Des(v)$ for class 1 immoralities. For each $u\sim v\in\cU_0\setminus \cU_1$ and any $w \in V\setminus\{u,v\}$, test if $u\not\CI v \mid w$. Then $u\not\CI v \mid w$ if and only if $w\in\Des(u)\cap\Des(v)$, i.e., $u,v\in R_w\subseteq\Anc(w)$. Finally update $R_w$ for all $w\in V$, where $R_w\leftarrow R_w\cap R_{w'}$ if $w'\in R_w$. (to show if: find the two directed paths to $w$, to show only if: consider the open path and any collider on it)
    \item iteratively identify class 2 immoralities by performing type 3 independence tests for all $u\in V$ and $u\sim v\in\cU_1$. remove $u\sim v\in \cU_1$ if it passes the tests. this terminates in $\cO(n^4)$ steps and finds all the class 2 immoralities. (to show termination: each time find one using at most $\cO(n^2)$ tests and there are at most $\cO(n^2)$ one, to show all are found: consider immorality pair $u\sim v\in\cU_1$ such that there is no immorality pair amongst $\Anc(u)\cap\Anc(v)$ \jj{need the formalized stuffs, ..... in fact I think the classes are not necessary for this argument})
\end{itemize}


==> backup/search.tex <==
\section{Search}

\begin{lemma}
    Let $A$ be such that $u \CI v~|~A$, then there exists a subset $B \subseteq A$ such that $u \CI v~|~B$ and $B \subseteq \Anc(u) \cup \Anc(v)$. Given set $A$, set $B$ satisfying the aforementioned properties can be found in polynomial number of independence tests.
\end{lemma}
\begin{proof}
     Consider the leaf node in $A$ and remove it; this preserves the independence relation between $u$ and $v$. We can keep removing the leaf nodes until the conditions of the lemma are satisfied. \jj{how do we get the leaf nodes?}
\end{proof}


==> content/results__Kiran_Shiragur_s_conflicted_copy_2024-02-02_.tex <==
\newcommand{\expt}[1]{\mathbb{E}\left[ #1\right]}
\newcommand{\findsrc}{\mathrm{FindSource}}
\newcommand{\src}{\mathrm{src}}
\newcommand{\Pt}{\mathcal{P}}
\newcommand{\iDes}[1]{\mathrm{iDes}(#1)}

\section{Results}
\label{sec:results}

Here we state all our main results of the paper. As discussed in the introduction, the main contribution of our work is in the recovery of ordering on a partition of the vertex set that is consistent with the ordering defined by the causal graph. In addition, our ordering several other nice properties which would help us recover the causal graph under some special but important cases. To help capture these properties, in the following we define the following characterization.

\begin{definition}
	Consider DAG $\cG$ on vertices $V$. A \emph{topological component graph (TCG)} representation of $\cG$ is a partition of $V$ into disjoint components $V_1,\dots,V_k$ and a directed acyclic graph $\cD$ between the components such that it satisfies
	\begin{itemize}
		\item \textbf{property of each component:} for each $i\in [k]$, there is $|\src(V_i)|=1$. Furthermore, if $|V_i|>1$, then $\cG[V_i]$ has at least one covered edge.
		\item \textbf{property of the graph between components:} $\cD$ is topologically ordered, i.e., $i\rightarrow j$ in $\cD$ only if $i<j$. It is also a consistent coarser representation of $\cG$ in the sense that:
		\begin{enumerate}
			\item if there is no edge $i\rightarrow j$ in $\cD$, then there is no edge from any vertex in $V_i$ to any vertex in $V_j$ in $\cG$,
			\item if there is an edge $i\to j$ in $\cD$, then there is $u\in V_i$ such that $u\in\Pa(\src(V_j))$.
		\end{enumerate}  
	\end{itemize}
\end{definition}
The second property in the above definition capture the consistent ordering and the first captures the some sense niceness of the TCG. The more formal description of the consistency of TCG is captured by the following result.
\begin{corollary}
	Let $\cG$ be a DAG and $\cD$ be its topological order, then for any valid topological ordering on the partition of the vertex set, there exists an ordering for the vertices within the each subset $V_{i}$ such that the resulting ordering will be a valid order for $\cG$.        
\end{corollary}

Note that if $|V_i|=1$, then TCG is actually the fully oriented graph and if $|V_i|>1$, then it means that there is a covered edge in this subset which requires additional interventional data to orient. An immediate remark from our definition of TCG is that, the number of subsets that have cardinality greater than 1, serve as a lower bound on the verification number, which is the number of internvetions needed to orient the whole graph. Based on this discussion, it is desirable to have partitions where subsets are of small size.

The main algorithmic contribution of our work is that we provide an efficient algorithm that performs at most polynomial number of independence tests and outputs a valid TCG of the hidden causal graph. 

\begin{theorem}\label{thm:main-1}
	Given observational data from a causal graph $\cG$, there exists a polynomial-time-running algorithm that performs at most $O(n^5)$ CI tests, and outputs a TCG representation of $\cG$.
	% a partition of the vertices into sets $V_{1},\dots V_{k}$ and a directed ayclic graph $G'$ on $k$ vertices corresponding to these sets such that,
	% \begin{enumerate}
		%     \item If $i \to j$  is an edge in the graph, then for all $u \in V_{i}$ and $v \in V_{j}$ we have $v \in \Des(u)$.
		%     \item For each ${i} \in [k]$, the $|\src(V_{i})|=1$. Furthermore, if $|V_{i}|>1$ then it has at least one covered edge.
		% \end{enumerate}
	%and interventional distributions corresponding to sets $\{I_{i} \}_{i=1}^{k}$
\end{theorem}

An immediate application of the above result is that, if the underlying causal graph has no covered edges, equivalently if its verification number is zero, then there exists a unique TCG which is the causal graph itself. Therefore in such a case, we recover the hidden causal graph with polynomial number of independence tests.

\begin{lemma}
	Given observational data from a hidden causal graph $\cG$ with verification number zero, we provide an efficient algorithm that performs at most polynomial number of independence tests and recovers the hidden underlying causal graph.
\end{lemma}

In addition to the above, we use our main theorem to also provide an analagous result in the presence of interventional data which is summarized in the following lemma.

\begin{lemma}
	Given observational and interventional data from a hidden causal graph $\cG$ which is sufficient to orient the whole causal graph, we provide an efficient algorithm that performs at most polynomial number of independence tests and recovers the hidden underlying causal graph.
\end{lemma}

\kk{compare with PC somewhere}

To the best of our knowledge, our main theorem and the other two derived results are the first of the kind which try to understand the information about the causal graph that can be recovered using polynomial number of independence tests.

We also quickly remark that, the last lemma states that we can recover causal graph in polynomial number of independence tests when we are provided with a verifying set. Although most of the algorithms require essential graph (which requires exponential tests in the first place) to output veryfying sets of small size, there are some randomized algorithms that output non-atomic verifying sets of small size. For instance, one such algorithm corresponds just picking a vertex independently with probability 1/2, and picking log n many independent subsets with high probabuilty will be verifying set. These interventions combined with our result provide recovers the causal graph with polynomial number of independence tests.

In light of this discussion, a very interesting open direction would be to find the approximately optimal verifying sets in polynomail number of independence tests. We will provide a discussion over this question in the final discussion section.

The main ingredient of our algorithm is a procedure which takes in a prefix subset and outputs a new set potentially of small size such that their union is still a prefix subset. The gaurantees of the prefix subset algorithm are summarized in the following theorem.
\kk{copy paste prefix subset result.}

\kk{may be make some remarks.}

To prove our main theorem we had to prove several other interesting results that we state below. We believe these results are quite general and may be applicable beyong the scope of this project. In the following we state two of the results one of which similar to v-structure statement and other to one of the Meek rules.

\begin{lemma}[Generalization of v-structure statement]\label{lemma:v-generalization}
	Let $S\subseteq V$ and $u,v,z \in V \backslash S$. If $u \CI v|S$ and $u \not \CI v|S \cup \{z \}$, then $u,v \not \in \Des[z]$.
\end{lemma}
The above lemma is analogous to v-structure statement in the sense that, if in addition to our conditions above is we are gauranteed that $u$ and $v$ are adjacent to $z$, then it would imply that the orientations on these edges will be $u \to z$ and $v \to z$ forming a v-strucutre. Such a v-structure would imply that $u,v \in \Pa(z)$. In the absence of the information about the adjajeney we can only show a weaker version of the v-strucutre statement in the sense that we can only gaurantee that $u$ and $v$ are not descendants of $z$. Our above lemma is tight as there exists a graph where the conditions of the lemma are met but $z$ is uncomporable to both $u$ and $v$. Example of such a graph is given below. 


\begin{lemma}[Generalization of Meek rule 1]\label{lem:general-meekrule-1}
	Let $S$ be a prefix subset. If $u,v$ and $w$ are such that $u \in S$, $v, w \not \in S$ and $u \not \CI v |S$ and $u \CI w|S\ \cup \{ v\}$ then $v \not \in \Des[w]$.
\end{lemma}
Similar to earlier discussion on v-structure related lemma, the above lemma is analogous to Meek rule 1. In Meek rule 1, with stronger conditions one could show that $v \in \Pa(w)$ but all we could show under mild conditions that $v$ is not a descendant of $w$.

In both the cases, one can show stronger statements when the adjaney between the vertices are known. However, adjancecies are the difficult to infer and are the bottleneck in achieving poly tests in causal discovery. Therefore our lemma statements show weaker relationships but do it with just constant tests. The most importatnt contribution of our work is in using these weaker relationships and yet constructing something meaningful out of it and in our algorithm we use these lemmas with several other nice properties to implement the prefix subset procedure, therefore the TCG algorithm.

\kk{Add image for both cases.}

\kk{Ingnore below this.}
\kk{Stating all the results here}
\begin{itemize}
    \item If the verification number if zero, can find the causal graph from the observational data in poly independence tests.
    \item Given observational data and atomic verifying set, can find the causal graph in poly independence tests.
    \item Generalization of to non-atomic verifying set. \kk{Haven't done this yet, might encounter new challenges.}
    \item All the above results are very significant compared to the PC algorithm. Compare it with that.
    \item Check if the given set is a verifying set can be solved in polynomial number of independence test?
    \item State results on how to find verifying intervention set where we do not need essential graph to begin with. \kk{We will use this result to}.
    \item State search problem as an open problem: given poly number of independence tests, how many interventions do we need to orient the whole graph?
    \item Another open problem: extending our results to latent variable setting.
\end{itemize}



\jj{The older description version is shorter: ``\emph{there is an edge $i\rightarrow j$ in $\cD$ if and only if $i<j$ and there is $u\in V_i$ such that $u\in\Pa(\src(V_j))$. Additionally, if there is no edge $i\rightarrow j$ in $\cD$, then there is no edge from any vertex in $V_i$ to $V_j$ in $\cG$.}'' -- however, i was not fully happy with it. essentially i want to say is it is consistent (no edge $\cD$ means no edge in $\cG$, edge $\cD$ means edge in $\cG$) and minimum (edge only when parents). then the topological thing $i<j$ is just for simplicity.}

Note that (1) TCG always exists. Consider the DAG itself, (2) if $\cG$ has no covered edge, then its only TCG representation is itself.

\jj{make a few illustrations}

\kk{To understand that the TCG catpures some meaningful information, we prove the following lemma.}


    



% \begin{theorem}
%     Given observational data from a causal graph $G[V,E]$, we can find a partition of the vertices into sets $V_{1},\dots V_{k}$ and a directed ayclic graph $G'$ on $k$ vertices corresponding to these sets such that,
%     \begin{enumerate}
%         \item If $i \to j$  is an edge in the graph, then for all $u \in V_{i}$ and $v \in V_{j}$ we have $v \in \Des(u)$.
%         \item For each ${i} \in [k]$, the $|\src(V_{i})|=1$. Furthermore, if $|V_{i}|>1$ then it has at least one covered edge.
%     \end{enumerate}
%     %and interventional distributions corresponding to sets $\{I_{i} \}_{i=1}^{k}$
% \end{theorem}

\subsection{Canonical Tests and Prefix Vertex Sets}

\jj{define the test we will do}





















==> plots/meek-rules.tex <==
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}
%
% R1
%
\node[draw, circle, inner sep=2pt] at (0,0) (R1a-before) {\small $a$};
\node[draw, circle, inner sep=2pt, right=of R1a-before] (R1b-before) {\small $b$};
\node[draw, circle, inner sep=2pt, above=of R1a-before](R1c-before) {\small $c$};
\draw[thick, -stealth] (R1c-before) -- (R1a-before);
\draw[thick] (R1a-before) -- (R1b-before);

\node[draw, circle, inner sep=2pt] at (3,0) (R1a-after) {\small $a$};
\node[draw, circle, inner sep=2pt, right=of R1a-after] (R1b-after) {\small $b$};
\node[draw, circle, inner sep=2pt, above=of R1a-after](R1c-after) {\small $c$};
\draw[thick, -stealth] (R1c-after) -- (R1a-after);
\draw[thick, -stealth] (R1a-after) -- (R1b-after);

\node[single arrow, draw, minimum height=2em, single arrow head extend=1ex, inner sep=2pt] at (2.2,0.75) (R1arrow) {};
\node[above=5pt of R1arrow] {\footnotesize R1};

%
% R2
%
\node[draw, circle, inner sep=2pt] at (6,0) (R2a-before) {\small $a$};
\node[draw, circle, inner sep=2pt, right=of R2a-before] (R2b-before) {\small $b$};
\node[draw, circle, inner sep=2pt, above=of R2a-before](R2c-before) {\small $c$};
\draw[thick, -stealth] (R2a-before) -- (R2c-before);
\draw[thick, -stealth] (R2c-before) -- (R2b-before);
\draw[thick] (R2a-before) -- (R2b-before);

\node[draw, circle, inner sep=2pt] at (9,0) (R2a-after) {\small $a$};
\node[draw, circle, inner sep=2pt, right=of R2a-after] (R2b-after) {\small $b$};
\node[draw, circle, inner sep=2pt, above=of R2a-after](R2c-after) {\small $c$};
\draw[thick, -stealth] (R2a-after) -- (R2c-after);
\draw[thick, -stealth] (R2c-after) -- (R2b-after);
\draw[thick, -stealth] (R2a-after) -- (R2b-after);

\node[single arrow, draw, minimum height=2em, single arrow head extend=1ex, inner sep=2pt] at (8.2,0.75) (R2arrow) {};
\node[above=5pt of R2arrow] {\footnotesize R2};

%
% R3
%
\node[draw, circle, inner sep=2pt] at (12,0) (R3d-before) {\small $d$};
\node[draw, circle, inner sep=2pt, above=of R3d-before](R3a-before) {\small $a$};
\node[draw, circle, inner sep=2pt, right=of R3a-before] (R3c-before) {\small $c$};
\node[draw, circle, inner sep=2pt, right=of R3d-before](R3b-before) {\small $b$};
\draw[thick, -stealth] (R3c-before) -- (R3b-before);
\draw[thick, -stealth] (R3d-before) -- (R3b-before);
\draw[thick] (R3c-before) -- (R3a-before) -- (R3d-before);
\draw[thick] (R3a-before) -- (R3b-before);

\node[draw, circle, inner sep=2pt] at (15,0) (R3d-after) {\small $d$};
\node[draw, circle, inner sep=2pt, above=of R3d-after](R3a-after) {\small $a$};
\node[draw, circle, inner sep=2pt, right=of R3a-after] (R3c-after) {\small $c$};
\node[draw, circle, inner sep=2pt, right=of R3d-after](R3b-after) {\small $b$};
\draw[thick, -stealth] (R3c-after) -- (R3b-after);
\draw[thick, -stealth] (R3d-after) -- (R3b-after);
\draw[thick] (R3c-after) -- (R3a-after) -- (R3d-after);
\draw[thick, -stealth] (R3a-after) -- (R3b-after);

\node[single arrow, draw, minimum height=2em, single arrow head extend=1ex, inner sep=2pt] at (14.2,0.75) (R3arrow) {};
\node[above=5pt of R3arrow] {\footnotesize R3};

%
% R4
%
\node[draw, circle, inner sep=2pt] at (18,0) (R4a-before) {\small $a$};
\node[draw, circle, inner sep=2pt, above=of R4a-before](R4d-before) {\small $d$};
\node[draw, circle, inner sep=2pt, right=of R4d-before] (R4c-before) {\small $c$};
\node[draw, circle, inner sep=2pt, right=of R4a-before](R4b-before) {\small $b$};
\draw[thick, -stealth] (R4d-before) -- (R4c-before);
\draw[thick, -stealth] (R4c-before) -- (R4b-before);
\draw[thick] (R4d-before) -- (R4a-before) -- (R4c-before);
\draw[thick] (R4a-before) -- (R4b-before);

\node[draw, circle, inner sep=2pt] at (21,0) (R4a-after) {\small $a$};
\node[draw, circle, inner sep=2pt, above=of R4a-after](R4d-after) {\small $d$};
\node[draw, circle, inner sep=2pt, right=of R4d-after] (R4c-after) {\small $c$};
\node[draw, circle, inner sep=2pt, right=of R4a-after](R4b-after) {\small $b$};
\draw[thick, -stealth] (R4d-after) -- (R4c-after);
\draw[thick, -stealth] (R4c-after) -- (R4b-after);
\draw[thick] (R4d-after) -- (R4a-after) -- (R4c-after);
\draw[thick, -stealth] (R4a-after) -- (R4b-after);

\node[single arrow, draw, minimum height=2em, single arrow head extend=1ex, inner sep=2pt] at (20.2,0.75) (R4arrow) {};
\node[above=5pt of R4arrow] {\footnotesize R4};

% Separating lines
% \draw[thick] (0,-1) -- (10.5,-1);
\draw[thick] (5.25,1.75) -- (5.25,-0.25);
\draw[thick] (11.25,1.75) -- (11.25,-0.25);
\draw[thick] (17.25,1.75) -- (17.25,-0.25);
\end{tikzpicture}
}
